ir_explain: a Python Library of Explainable IR Methods

While recent advancements in Neural Ranking Models have resulted in significant improvements over traditional statistical retrieval models, it is generally acknowledged that the use of large neural architectures and the application of complex language models in Information Retrieval (IR) have reduced the transparency of retrieval methods. Consequently, Explainability and Interpretability have emerged as important research topics in IR. Several axiomatic and post-hoc explanation methods, as well as approaches that attempt to be interpretable-by-design, have been proposed. This article presents \irexplain, an open-source Python library that implements a variety of well-known techniques for Explainable IR (ExIR) within a common, extensible framework. \irexplain supports the three standard categories of post-hoc explanations, namely pointwise, pairwise, and listwise explanations. The library is designed to make it easy to reproduce state-of-the-art ExIR baselines on standard test collections, as well as to explore new approaches to explaining IR models and methods. To facilitate adoption, \irexplain is well-integrated with widely-used toolkits such as Pyserini and \irdatasets.

==> code-listing/listing-pyterrier-experiment.tex <==
\begin{listing}[tb]
    \lstinputlisting[
        firstline=2,
    ]{listing-pyterrier-experiment.py}
    \caption{Example of an experiment returning pairwise axiom preferences with retrieval models passed in a list.}
    \label{listing-pyterrier-experiment}
\end{listing}


==> design/design-specs.tex <==
 % LirmePointwiseExplainer(model, corpus_path = "../../../", indexer = "no-index")
 % index_path / corpus_path = "" and indexer = "pyserini"
 % index_path / corpus_path = "" and indexer = "pyterrier"

- Deadline  18 Feb, 4 Feb -- abstract submission deadline

TODO 

- New redesign for the entire pipeline
- Write the draft in this format
- maybe we can add one probing based approach and one IBD approach

Small TODO items:
1. Move metrics.py to eval folder
2. Add descriptors for all classes and methods
3. logging setup
4. Revisit some (be very specific to it) part and clean up 
5. Remove print statements from the code, maybe logger? or something else? 



==> how-extensible.tex <==
\subsection{How extensible is \irexplain module?}
\textcolor{red}{mainly to articulate what are the components comes for free to any users of \irexplain. Just like ir-axiom, you can define easily any new axiom, what are the components we are providing here?  }
-- mainly the utils, Perturbation classes, Evaualtion components
-- different explanation classes to start with 
-- different perturbation component
-- diverse analysis with \irexplain robust 

